B/Surf: Interactive B\'ezier Splines on Surfaces

B\'ezier curves provide the basic building blocks of graphic design in 2D. In this paper, we port B\'ezier curves to manifolds. We support the interactive drawing and editing of B\'ezier splines on manifold meshes with millions of triangles, by relying on just repeated manifold averages. We show that direct extensions of the De Casteljau and Bernstein evaluation algorithms to the manifold setting are fragile, and prone to discontinuities when control polygons become large. Conversely, approaches based on subdivision are robust and can be implemented efficiently. We define B\'ezier curves on manifolds, by extending both the recursive De Casteljau bisection and a new open-uniform Lane-Riesenfeld subdivision scheme, which provide curves with different degrees of smoothness. For both schemes, we present algorithms for curve tracing, point evaluation, and point insertion. We test our algorithms for robustness and performance on all watertight, manifold, models from the Thingi10k repository, without any pre-processing and with random control points. For interactive editing, we port all the basic user interface interactions found in 2D tools directly to the mesh. We also support mapping complex SVG drawings to the mesh and their interactive editing.

==> 03_preliminaries.tex <==
% !TEX root = bsurf.tex
\section{Preliminaries}
\label{sec:prelim}
We briefly review basic definitions and properties about: B\'ezier curves in the Euclidean settings; geodesics on manifold surfaces and meshes; and weighted averages on manifolds. 

\subsection{B\'ezier Curves in the Euclidean Setting}
\label{sub:bezier-euclidean}
For the contents of this section, we refer to \cite{Farin2001,Salomon:2006wp}. 

A B\'ezier curve of degree $k$ is defined by a set of $k+1$ control points $P_0,\ldots, P_k\in\mathbb{R}^d$.
The polyline $\Pi^k$ connecting such points in the given order is called the \emph{control polygon} of the curve. 
The curve can be described by a polynomial parametric function of degree $k$, which, without lack of generality, we assume to be defined in $[0,1]$ %and have constant speed
$$\mathbf{b}^k : [0,1]\longrightarrow \mathbb{R}^d.$$
The B\'ezier curve interpolates $P_0$ and $P_k$ and it is tangent to the control polygon $\Pi^k$ at such two points. 

\subsubsection{The De Casteljau construction.}
\label{sub:decasteljau}
A point on a B\'ezier function at parameter $t\in[0,1]$ can be evaluated as $\mathbf{b}^k(t) = \mathbf{b}_0^k(t)$, according to the following recursive definition:
\begin{equation}
\label{eq:decasteljau}
\begin{array}{l}
\mathbf{b}_i^0(t)=P_i\\
\mathbf{b}_i^r(t) = (1-t)\mathbf{b}_i^{r-1}(t) + t \mathbf{b}_{i+1}^{r-1}(t)
\end{array}
\end{equation}
for $r=1,\ldots, k$ and $i=0,\ldots, k-r$.
%Point evaluation with this construction requires computing $k(k-1)$ convex averages between pairs of control points for a given value of $t$. 
The construction for a cubic curve is depicted in Figure \ref{fig:decasteljau}(a).

\subsubsection{The Bernstein definition.}
\label{sub:bernstein}
The same curve is defined by expression
\begin{equation}
\label{eq:bernstein}
\mathbf{b}^k(t) = \sum_{i=0}^k B_i^k(t) P_i %\hspace{1cm} t\in [0,1]
\end{equation}
where the $B_i^k(t)$ are the Bernstein basis polynomials of degree $k$
\[B_i^k(t) = \binom{k}{i} t^i(1-t)^{n-i}.\]
%In this case, point evaluation for a given $t$ requires just one convex average of the $k+1$ control points. 

\subsubsection{Subdivision by degree elevation.}
\label{sub:subdegree}
The curve $\mathbf{b}^k$ can be rewritten as a B\'ezier curve of degree $k+1$ on a control polygon $\Pi^{k+1}$ with control points
\begin{equation}
\label{eq:degel}
P_i^{k+1} = \frac{i}{k+1} P_{i-1}+\left(1-\frac{i}{k+1}\right)P_i, \hspace{1cm} i=0,\ldots,k+1.
\end{equation}
The repeated application of degree elevation generates a sequence of control polygons $\Pi_{de}^N$ that converges to the B\'ezier curve for $N\rightarrow\infty$. 
%However, the cost of generating a polygon with $N$ segments, for $N>>k$, requires $O(N^2)$ evaluations of the expression above.\footnote{A more compact expression that computes the $N$ points in $O(kN)$ is possible, but it is not useful for our purposes, as explained in Section \ref{sec:????}} 

\subsubsection{Recursive De Casteljau bisection.}
\label{sub:subDC}
One step of De Casteljau evaluation subdivides the control polygon $\Pi$ into two control polygons $\Pi_L$ and $\Pi_R$, as illustrated in Figure \ref{fig:decasteljau}(b). 
The middle point $\mathbf{b}^k(t)$ lies on the curve and becomes an endpoint of both $\Pi_L$ and $\Pi_R$. 
The recursive application of this procedure for $t=1/2$ defines a sequence of subdivision polygons $\Pi_{DC}^N$, each consisting of all endpoints of the control polygons, which converges to the B\'ezier curve for $N\rightarrow\infty$.  

\subsubsection{Non-uniform Lane-Riesenfeld subdivision.}
\label{app:subLR}
A B-spline of degree $k$ (order $k+1$) with the same control polygon $\Pi^k$ and knot vector $(00\ldots011\ldots1)$, where the $0$ and $1$ are repeated $k+1$ times, defines the same curve $\mathbf{b}^k$.
The compact expression of such a B-spline in fact reduces to the Bernstein form of Eq.~\ref{eq:bernstein}. 
Repeated knot insertion at the midpoint of all non-zero intervals in the knot vector produces a sequence of open uniform B-splines, whose control polygons $\Pi_{LR}^N$ converge to the B\'ezier curve for $N\rightarrow\infty$.
This subdivision curve follows a non-uniform Lane-Riesenfeld scheme \cite{Lane:dq} (\emph{LR} in the sequel). 
% where the central segments follows the standard LR rule for odd and even control points, while boundary rules are necessary to keep the endpoints of the curve fixed. 
The subdivision matrices with B\'ezier end conditions are described in \cite{Cashman:2007jh}.
We report here the subdivision masks for a cubic curve:
\begin{equation}
\label{eq:LR}
\begin{array}{l}
\hspace{-6pt} \left. \begin{array}{l}
P_{2j}^N=\frac{1}{2}P_j^{N-1}+\frac{1}{2}P_{j+1}^{N-1}\\[5pt]
P_{2j+1}^N=\frac{1}{8}P_j^N+\frac{3}{4}P_{j+1}^N+\frac{1}{8}P_{j+2}^N
\end{array} \hspace{0.5cm} \right\}  j=4...2^N-2\\[12pt]
P_0^N=P_0 \\[5pt]
P_1^N=\frac{1}{2}P_0^{N-1}+\frac{1}{2}P_1^{N-1} \\[5pt]
P_2^N=\frac{3}{4}P_1^{N-1}+\frac{1}{4}P_2^{N-1} \\[5pt]
P_3^N=\frac{3}{16}P_1^{N-1}+\frac{11}{16}P_2^{N-1}+\frac{2}{16}P_3^{N-1} \\[5pt]
P_{2^N-1}^N=\frac{2}{16}P_{\frac{2^N-2}{2}}^{N-1}+\frac{11}{16}P_{2^{N-1}}^{N-1}+\frac{3}{16}P_{\frac{2^N+2}{2}}^{N-1} \\[5pt]
P_{2^N}^N=\frac{1}{4}P_{2^{N-1}}^{N-1}+\frac{3}{4}P_{\frac{2^{N}+2}{2}}^{N-1} \\[5pt]
P_{2^N+1}^N=\frac{1}{2}P_{\frac{2^N+2}{2}}^{N-1}+\frac{1}{2}P_{\frac{2^N+4}{2}}^{N-1} \\
P_{2^N+2}^N=P_3 \\
\end{array}
\end{equation}
where $N$ is the level of subdivision, which contains the points $P_i^N$ for $i=0,\ldots, 2^N+2$.
Note that the first two rows in Scheme \ref{eq:LR} give the uniform LR scheme, which is applied to all central points, while the remaining rows set the end conditions, to keep the endpoints of the curve fixed. 
For a generic B\'ezier curve of degree $k$, there will be $2(k+1)$ stencils for end conditions. %, the first and the last setting trivially that the endpoints are fixed. 

Note also that the LR scheme is given here in compact form, while its classical definition assumes one step of averaging, followed by $k-1$ steps of smoothing. 
According to the latter, all averages that involve more than two control points can be rewritten as repeated averages between pairs of points. 
For instance, the second row in (\ref{eq:LR}) can be rewritten as  
\[
\begin{array}{ll}
\bar{P}_j^N=\frac{1}{2}(P_j^{N-1}+P_{j+1}^{N-1}); & \bar{P}_{j+1}^N=\frac{1}{2}(P_{j+1}^{N-1}+P_{j+2}^{N-1});\\ 
\hat{P}_j^N=\frac{1}{2}(\bar{P}_j^N+P_{j+1}^{N-1}); & \hat{P}_{j+1}^N=\frac{1}{2}(P_{j+1}^{N-1}+\bar{P}_{j+1}^N);\\ 
P_{2j}^N=\frac{1}{2}(\hat{P}_j^N+\hat{P}_{j+1}^N) & \\
\end{array}
\]
and likewise for rows 6 and 7. 
This fact will be relevant for our extension of this scheme to the manifold setting. 

\bigskip
\bigskip
Finally, notice that the three subdivision schemes presented above generate three different subdivision sequences $\Pi_{de}^N$,  $\Pi_{DC}^N$,  $\Pi_{LR}^N$, which all converge to the same B\'ezier curve. 







 
 \subsection{Weighted Averages on Surfaces}
 \label{sub:weightedave}





